Security and Privacy: Key Requirements for Molecular Communication in Medicine and Healthcare

Molecular communication (MC) is an emerging paradigm that enables data transmission through biochemical signals rather than traditional electromagnetic waves. This approach is particularly promising for environments where conventional wireless communication is impractical, such as within the human body. However, security and privacy pose significant challenges that must be addressed to ensure reliable communication. Moreover, MC is often event-triggered, making it logical to adopt goal-oriented communication strategies, similar to those used in message identification. This work explores secure identification strategies for MC, with a focus on the information-theoretic security of message identification over Poisson wiretap channels (DT-PWC).

==> Figures/MC.tex <==
\tikzset{semicircle/.pic = {
    \draw (0:3) -- (0:4);
    \draw [thick, xshift = .5cm, yshift = .5cm](0*40:4) arc (90:270:.5);
}}
% ---
\tikzset{triangle/.pic = {
    \draw (0:3) -- (0:4);
    \draw [thick] (0:4) -- ([xshift = .5cm, yshift = .5cm]0:4);
    \draw [thick] (0:4) -- ([xshift = .5cm, yshift = -.5cm]0:4);
}}
% ---
\tikzset{square/.pic = {
    \draw (0*40:3) -- (0*40:4);
    \draw [thick] (0:4) -- ([xshift = 0cm, yshift = .5cm]0:4);
    \draw [thick] (0:4) -- ([xshift = 0cm, yshift = -.5cm]0:4);
    \draw [thick] ([xshift = 0cm, yshift = +.5cm]0:4) -- ([xshift = .5cm, yshift = +.5cm]0:4);
    \draw [thick] ([xshift = 0cm, yshift = -.5cm]0:4) -- ([xshift = .5cm, yshift = -.5cm]0:4);
}}

\tikzset{triangle/.style = { isosceles triangle,
    isosceles triangle apex angle=60,
    draw,fill= red!50, minimum size = .1cm, rotate=90,
    inner sep=0pt
    }}
% ---
% \tikzset{RX/.pic = {
    % \foreach \x [count=\p] in {0,...,11} {
    % \node [shape = circle, fill = black, scale = 0.3] (\p) at (-\x*40:2) {};},
    % \foreach \x [count=\p] in {0,3,6} {\path[rotate = -\x*40, transform shape] pic{semicircle};}
    % \foreach \x [count=\p] in {1,4,7} {\path[rotate = -\x*40, transform shape] pic{triangle};}
    % \foreach \x [count=\p] in {2,5,8} {\path[rotate = -\x*40, transform shape] pic{square};}
    % \draw (1) arc (0:360:2);
% }}
% ---
\begin{tikzpicture}[scale=0.41]
    % Around TX
    % \pgfmathsetseed{1125}
    \pgfmathsetseed{53}
    \foreach \p in {1,...,15}{
    % \draw [fill = orange] (3*rand-19 , 3*rand+.5) circle (0.1);
    % \draw [fill = blue] (3*rand-19.5 , 3*rand) rectangle ++ (.17,.17);
    % \node[triangle] at (3*rand-18.5 , 3*rand+.5) {};
    \draw [fill = orange] (1.4*rand-20 , 1.4*rand) circle (0.1);
    \node[triangle] at (2.1*rand-20 , 2.2*rand) {};
    \draw [fill = blue] (2.5*rand-19.5 , 2.5*rand) rectangle ++ (.17,.17);
    }
    % Around RX
    \node[triangle] at (-4.1,-1.4) {};
    \node[triangle] at (3.28,-3) {};
    
    \draw [fill = blue] (3.24,3) rectangle ++ (.17,.17);
    \draw [fill = blue] (-4.1,1.4) rectangle ++ (.17,.17);

    \draw [fill = orange] (-2,3.65) circle (0.1);
    \draw [fill = orange] (-2.3,3.59) circle (0.1);
    
    % \node[isosceles triangle,
    % isosceles triangle apex angle=60,
    % draw,fill=teal!10,
    % minimum size =1cm, rotate=90] (T60) at (-20,0){};
    
    \draw [fill = gray!10, fill opacity = 1] (-20,0) circle (0.7 cm);
    \draw [thick] (-20,0) circle (.7cm);
    \node [] at (-20,0) {\text{TX}};
    % RX
    \foreach \x [count=\p] in {0,...,11} {
    \node [shape = circle, fill = cyan, scale = 0.3] (\p) at (-\x*40:3) {};}
    \foreach \x [count=\p] in {0,3,6} {\path[rotate = -\x*40, transform shape] pic{semicircle};}
    \foreach \x [count=\p] in {1,4,7} {\path[rotate = -\x*40, transform shape] pic{triangle};}
    \foreach \x [count=\p] in {2,5,8} {\path[rotate = -\x*40, transform shape] pic{square};}
    \draw (1) arc (0:360:3);
    \draw [fill = yellow!10, fill opacity = 1] (0,0) circle (3 cm);
    \node [] at (0,0) {\text{RX}};
    %
\end{tikzpicture}
